Towards single integrated spoofing-aware speaker verification embeddings

This study aims to develop a single integrated spoofing-aware speaker verification (SASV) embeddings that satisfy two aspects. First, rejecting non-target speakers' input as well as target speakers' spoofed inputs should be addressed. Second, competitive performance should be demonstrated compared to the fusion of automatic speaker verification (ASV) and countermeasure (CM) embeddings, which outperformed single embedding solutions by a large margin in the SASV2022 challenge. We analyze that the inferior performance of single SASV embeddings comes from insufficient amount of training data and distinct nature of ASV and CM tasks. To this end, we propose a novel framework that includes multi-stage training and a combination of loss functions. Copy synthesis, combined with several vocoders, is also exploited to address the lack of spoofed data. Experimental results show dramatic improvements, achieving a SASV-EER of 1.06% on the evaluation protocol of the SASV2022 challenge.

==> Old_intro.tex <==
\jee{Automatic speaker verification (ASV) is designed as a means of biometric in its natural formulation. 
To be applied in real world scenarios it has to have the capability to reject both bona fide non-target speakers' inputs as well as target speaker's spoofed inputs.
However, because the technology was not yet matured, the ASV research community had no choice but to leave spoofing scenario out of the table. 
Initially works on ASV even removed phonetic variabilities and focused on text-dependent scenario~\cite{}.}

\jee{
ASV task has experienced a rapid development in the last few decades. 
Nowadays, state-of-the-art ASV systems~\cite{kinnunen2010overview} offer exceptional reliability across diverse scenarios and domains~\cite{zhang2022mfa,jung22_interspeech,chen2022large}.
Nonetheless, their vulnerabilities to spoofing and deepfake attacks are well acknowledged.
}
%Recent developments in automatic speaker verification (ASV)~\cite{kinnunen2010overview} have emerged as a promising means of verifying users' identities. 
% Although ASV systems can be utilised in various applications for biometric authentication, it is important to consider the possibility of spoofing attacks, wherein the ASV system can be deceived using manipulated samples generated through speech synthesis or voice conversion. 
%While today's state-of-the-art 
%ASV systems~\cite{kinnunen2010overview} %can now robustly distinguish whether an input utterance is from a target speaker 
%offer exceptional reliability across diverse scenarios and domains~\cite{zhang2022mfa,jung22_interspeech,chen2022large},
%However, it has been reported that these state-of-the-art ASV systems are highly 
%their vulnerabilities to spoofing and deepfake attacks are well acknowledged. 
Such malicious attacks are generated using text-to-speech and voice conversion algorithms, for instance, in order to deceive an ASV system and provoke an increased rate of false positives.
As a result, the development of spoofing and deepfake detection systems, known as countermeasures (CM) has attracted considerable research interest~\cite{kinnunen2017asvspoof,wang2020asvspoof,yamagishi21_asvspoof}.
The majority of CM systems take the form of standalone, auxiliary binary classifiers and have the role of determining whether a given utterance is bona fide (i.e., genuine) or spoofed.

% Typical CM systems operate as standalone systems and the ASV scenario is merely provided as a fixed condition (ASV scores) for calculating the tandem DCF error. 
% Hence, CM systems' effectiveness can be influenced by the ASV system adopted, when applied in real-world scenarios.
% Under these circumstances, the CM system can exhibit promising results; however, its effectiveness may be limited when applied in real-world scenarios depending on the ASV system's performance.

The first Spoofing-Aware Speaker Verification (SASV) challenge~\cite{jung2022sasv} was held in 2022 to promote research into the joint optimisation of ASV and CM, receiving widespread attention in this area with 53 registered participants. 
The goal was to recover the original objective of ASV, by becoming {\em spoofing-aware}, expanding the definition of the task.
% Most participants employed fusion systems based on given baseline systems and achieved an equal error rate (EER) of up to 0.13\% on the evaluation protocol, ASVspoof2019LA evaluation set~\cite{wang2020asvspoof}. 
However, most participants employed fusions leveraging two independent pre-trained systems: ASV and CM. 
Fusion was explored in diverse levels, embedding, score, or decision~\cite{zhang2022probabilistic, lin2022clips, dku2022sasv, hyu_sasv_2022}.% and the winning team~\cite{alenin2022subnetwork} achieved an equal error rate (EER) of 0.13\% on the ASVspoof2019LA evaluation protocol~\cite{wang2020asvspoof}. 
While a few participants explored end-to-end (E2E) approaches, training a single integrated SASV embedding from scratch or fully E2E SASV systems following the spirit of \cite{shim2020integrated,li2020joint,todisco2018integrated}, they significantly underperformed compared to the simpler fusion methods~\cite{kang2022end, teng2022sa}. 
We argue that this is a somewhat middle phase, somewhere between the integration phase of conventional ASV becoming an SASV. 

These results are analysed to be a result of two factors. 
First, the data, enough to train an SASV embedding from scratch, lacks. 
Second, ASV and CM are fundamentally distinct tasks; thus, they require different types of information to be performed. 
For instance, in ASV, a network may be trained to differentiate between individuals by focusing on their voice within the entire utterance, whereas, in the case of CM, a model may be trained to concentrate on noise or acoustic characteristics within a silent section~\cite{muller2021speech, mari2022sound}.
Recent studies on the joint-optimisation of ASV and CM~\cite{ge2022joint,ge2023joint} demonstrated the potential of integrated joint-training and, it also showed that the lack of speakers in training data degrade the ASV performance. The potential for joint optimisation to exploit the the synergy between ASV and CM sub-systems given the availability of a larger number of speakers in training data. 
This line of research, training a single integrated SASV embeddings is in its preliminary stage. 
Nevertheless, we argue that this simplifying strategy is clearly worthwhile of further studies because, for ASV to be more applied in real world applications, the scope of the task should be extended to cover spoofed inputs as well without employing additional CM models. The data and adequate training strategies would be the key.% and single integrated SASV embeddings without using pre-trained speaker and CM embeddings model is challenging and may necessitate careful and precise adjustments.

%\input{nickIntro}

The goal of this paper is to further push the performance of a single integrated SASV embedding so that it demonstrates competitive performance compared to the existing fusion techniques. 
For this purpose, our proposals in this paper are threefold, where two in front concentrate on the lack of data, and the last focuses on  delicate training techniques:
\begin{itemize}
    \item we propose and explore diverse multi-stage training schemes;
    \item we adopt {\em copy synthesis}, a spoofed data generation technique, for the multi-stage training;
    \item we propose to train the SASV embedding extractor using a combination of multiple objective functions.
\end{itemize}

The proposed multi-stage training scheme consists of either two or three phases, leveraging two types of pre-training phases correspondingly. Both pre-training techniques are devised to complement the lack of data to train a single integrated SASV embedding. 
Phase 1 utilises VoxCeleb2~\cite{chung2018voxceleb2}, a large-scale speaker recognition dataset. Whereas phase 2
involves a copy-synthesis technique to generate a massive amount of spoofed data by hypothesising an ideal acoustic model for speech synthesis and generating using diverse vocoders. Phase 3 utilised in-domain ASVspoof2019 LA training data for fine-tuning.
The proposed combinations of objective functions are used in both phase 2 and 3 which employs contrastive learning as well as one of the two types of identification losses that we explore.

We explored two recent deep neural network (DNN) architectures: selective kernel attention based time delay neural network (SKA-TDNN)~\cite{mun2023frequency} and multi-scale feature aggregation conformer (MFA-Conformer)~\cite{zhang2022mfa}. For the MFA-Conformer, we employ the convolution sub-sampling rate 1/2 version of~\cite{zhang2022mfa}.
Through extensive experiments, we confirm relative improvements in the performance of single integrated SASV system where the best performing configuration demonstrates a SASV-EER of 1.19\% on the SASV evaluation protocol.



% \jee{Automatic speaker verification (ASV) is designed as a means of biometric in its natural formulation. 
% To be applied in real world scenarios it has to have the capability to reject both bona fide non-target speakers' inputs as well as target speaker's spoofed inputs.
% However, because the technology was not yet matured, the ASV research community had no choice but to leave spoofing scenario out of the table. 
% Initially works on ASV even removed phonetic variabilities and focused on text-dependent scenario~\cite{}.}

% \jee{
% ASV task has experienced a rapid development in the last few decades. 
% Nowadays, state-of-the-art ASV systems~\cite{kinnunen2010overview} offer exceptional reliability across diverse scenarios and domains~\cite{zhang2022mfa,jung22_interspeech,chen2022large}.
% Nonetheless, their vulnerabilities to spoofing and deepfake attacks are well acknowledged.
% }
% %Recent developments in automatic speaker verification (ASV)~\cite{kinnunen2010overview} have emerged as a promising means of verifying users' identities. 
% % Although ASV systems can be utilised in various applications for biometric authentication, it is important to consider the possibility of spoofing attacks, wherein the ASV system can be deceived using manipulated samples generated through speech synthesis or voice conversion. 
% %While today's state-of-the-art 
% %ASV systems~\cite{kinnunen2010overview} %can now robustly distinguish whether an input utterance is from a target speaker 
% %offer exceptional reliability across diverse scenarios and domains~\cite{zhang2022mfa,jung22_interspeech,chen2022large},
% %However, it has been reported that these state-of-the-art ASV systems are highly 
% %their vulnerabilities to spoofing and deepfake attacks are well acknowledged. 
% Such malicious attacks are generated using text-to-speech and voice conversion algorithms, for instance, in order to deceive an ASV system and provoke an increased rate of false positives.
% As a result, the development of spoofing and deepfake detection systems, known as countermeasures (CM) has attracted considerable research interest~\cite{kinnunen2017asvspoof,wang2020asvspoof,yamagishi21_asvspoof}.
% The majority of CM systems take the form of standalone, auxiliary binary classifiers and have the role of determining whether a given utterance is bona fide (i.e., genuine) or spoofed.

% % Typical CM systems operate as standalone systems and the ASV scenario is merely provided as a fixed condition (ASV scores) for calculating the tandem DCF error. 
% % Hence, CM systems' effectiveness can be influenced by the ASV system adopted, when applied in real-world scenarios.
% % Under these circumstances, the CM system can exhibit promising results; however, its effectiveness may be limited when applied in real-world scenarios depending on the ASV system's performance.

% The first Spoofing-Aware Speaker Verification (SASV) challenge~\cite{jung2022sasv} was held in 2022 to promote research into the joint optimisation of ASV and CM, receiving widespread attention in this area with 53 registered participants. 
% The goal was to recover the original objective of ASV, by becoming {\em spoofing-aware}, expanding the definition of the task.
% % Most participants employed fusion systems based on given baseline systems and achieved an equal error rate (EER) of up to 0.13\% on the evaluation protocol, ASVspoof2019LA evaluation set~\cite{wang2020asvspoof}. 
% However, most participants employed fusions leveraging two independent pre-trained systems: ASV and CM. 
% Fusion was explored in diverse levels, embedding, score, or decision~\cite{zhang2022probabilistic, lin2022clips, dku2022sasv, hyu_sasv_2022}.% and the winning team~\cite{alenin2022subnetwork} achieved an equal error rate (EER) of 0.13\% on the ASVspoof2019LA evaluation protocol~\cite{wang2020asvspoof}. 
% While a few participants explored end-to-end (E2E) approaches, training a single integrated SASV embedding from scratch or fully E2E SASV systems following the spirit of \cite{shim2020integrated,li2020joint,todisco2018integrated}, they significantly underperformed compared to the simpler fusion methods~\cite{kang2022end, teng2022sa}. 
% We argue that this is a somewhat middle phase, somewhere between the integration phase of conventional ASV becoming an SASV. 

% These results are analysed to be a result of two factors. 
% First, the data, enough to train an SASV embedding from scratch, lacks. 
% Second, ASV and CM are fundamentally distinct tasks; thus, they require different types of information to be performed. 
% For instance, in ASV, a network may be trained to differentiate between individuals by focusing on their voice within the entire utterance, whereas, in the case of CM, a model may be trained to concentrate on noise or acoustic characteristics within a silent section~\cite{muller2021speech, mari2022sound}.
% Recent studies on the joint-optimisation of ASV and CM~\cite{ge2022joint,ge2023joint} demonstrated the potential of integrated joint-training and, it also showed that the lack of speakers in training data degrade the ASV performance. The potential for joint optimisation to exploit the the synergy between ASV and CM sub-systems given the availability of a larger number of speakers in training data. 
% This line of research, training a single integrated SASV embeddings is in its preliminary stage. 
% Nevertheless, we argue that this simplifying strategy is clearly worthwhile of further studies because, for ASV to be more applied in real world applications, the scope of the task should be extended to cover spoofed inputs as well without employing additional CM models. The data and adequate training strategies would be the key.% and single integrated SASV embeddings without using pre-trained speaker and CM embeddings model is challenging and may necessitate careful and precise adjustments.

% %\input{nickIntro}

% The goal of this paper is to further push the performance of a single integrated SASV embedding so that it demonstrates competitive performance compared to the existing fusion techniques. 
% For this purpose, our proposals in this paper are threefold, where two in front concentrate on the lack of data, and the last focuses on  delicate training techniques:
% \begin{itemize}
%     \item we propose and explore diverse multi-stage training schemes;
%     \item we adopt {\em copy synthesis}, a spoofed data generation technique, for the multi-stage training;
%     \item we propose to train the SASV embedding extractor using a combination of multiple objective functions.
% \end{itemize}

% The proposed multi-stage training scheme consists of either two or three phases, leveraging two types of pre-training phases correspondingly. Both pre-training techniques are devised to complement the lack of data to train a single integrated SASV embedding. 
% Phase 1 utilises VoxCeleb2~\cite{chung2018voxceleb2}, a large-scale speaker recognition dataset. Whereas phase 2
% involves a copy-synthesis technique to generate a massive amount of spoofed data by hypothesising an ideal acoustic model for speech synthesis and generating using diverse vocoders. Phase 3 utilised in-domain ASVspoof2019 LA training data for fine-tuning.
% The proposed combinations of objective functions are used in both phase 2 and 3 which employs contrastive learning as well as one of the two types of identification losses that we explore.

% We explored two recent deep neural network (DNN) architectures: selective kernel attention based time delay neural network (SKA-TDNN)~\cite{mun2023frequency} and multi-scale feature aggregation conformer (MFA-Conformer)~\cite{zhang2022mfa}. For the MFA-Conformer, we employ the convolution sub-sampling rate 1/2 version of~\cite{zhang2022mfa}.
% Through extensive experiments, we confirm relative improvements in the performance of single integrated SASV system where the best performing configuration demonstrates a SASV-EER of 1.19\% on the SASV evaluation protocol.

==> Old_section2.tex <==
\section{Multi-stage training scheme}
%\label{sec:multistage}
% The proposed training scheme includes between one to three phases, which consist of either of the two techniques to be explained in Sections \ref{ssec:sid} and \ref{ssec:cs}, or adopts both of them. 
Figure~\ref{fig:SASV} illustrates the overall proposed SASV framework. As shown in Figure~\ref{fig:SASV} training scheme is divided into three stages: speaker identification-based pre-training, multi-task training with copy-synthesis data, and end-to-end SASV fine-tuning. Each training stage is defined in the following sub-sections.

\subsection{Stage~1: Speaker identification-based pre-training}
\label{ssec:sid}
In order to compensate for the lack of data to train a single SASV system, VoxCeleb2~\cite{chung2018voxceleb2}, a large-scale speaker recognition dataset can be utilised. VoxCeleb2 development data only contains bona fide utterances from ~6k speakers. 
%In stage~1, the SASV embedding network is pre-trained on VoxCeleb data by optimising the equal-weighted summation of the AAM softmax~\cite{deng2019arcface} and the angular prototypical~\cite{chung2020defence} objective functions.
After pre-training stage, SASV embeddings are fine-tuned with both bona fide and spoofed utterances in stage~2.

\subsection{Stage~2: Copy synthesis training}
\label{ssec:cs}
Training data generated from a variety of text-to-speech (TTS) synthesis and voice conversion (VC) algorithms, is a prerequisite for constructing single integrated SASV models. Nonetheless, building various TTS and VC systems is a technically demanding and time-consuming process. It also requires high-quality training data. To avoid this, a recent study~\cite{Wang2023a} explored the neural network based vocoders to do copy-synthesis on bon fide utterances to generate spoofed data.
We used a similar idea to generate the copy-synthesis of VoxCeleb2 and ASVspoof 2019 LA training dataset. We employ four different types of neural vocoders as described in~\cite{Wang2023a}: HiFiGAN~\cite{Kong2020}, WaveGlow~\cite{prenger2018waveglow}, neural source-filter model (NSF) \cite{wang2018neural}, and NSF with a HiFiGAN discriminator. A vocoder takes acoustic features such as F0 and mel spectrogram as input and produces the speech waveforms.\\

While the acoustic features in TTS and VC are predicted from acoustic models given input text or source speech, for copy-synthesis, we extract (i.e., copy) the acoustic features from a target waveform and reconstruct (i.e., synthesise) the waveform.  Even though the copy-synthesised waveforms cannot encode the artefacts caused by acoustic models, they capture the vocoder's artefacts that might present in the spoofed data from the TTS and VC systems. The copy-synthesis data was found to be effective for spoofing CM~\cite{wu2013synthetic,Saratxaga2016,Wang2023a, sun2023exposing}. This set of vocoders covers flow, GAN, and differentiable digital signal processing techniques \cite{engel2020ddsp}. Furthermore, they generate waveforms at a real-time speed, making them ideal for copy-synthesis on a large data set. We use the copy synthesised data combined with corresponding bona fide data in stage~2. The model is trained using a combination of contrastive and identification loss functions described in Section~\ref{sec:loss}.

% \subsection{Phase 3: fine-tuning}
\subsection{Stage~3: Fine-tuning}
\label{ssec:ft}
In stage~3, we perform fine-tuning using in-domain bona fide and spoofed data from ASVspoof 2019 LA training dataset to improve generalisation. Stage~3 uses a similar training scheme and objective loss functions as stage~2.

This phase adopts the identical training mechanism to phase 2: we use the combination of different objective functions which  detailed in Section~\ref{sec:loss}.

We employ four types of neural vocoders released by \cite{Wang2023a}: HiFiGAN \cite{Kong2020}, WaveGlow \cite{prenger2018waveglow}, neural source-filter model (NSF) \cite{wang2018neural}, and NSF with a HiFiGAN discriminator.
The task can become more challenging if the original (i.e., bona fide) data is not clean; the majority of TTS and VC algorithms assume high-quality clean data.
they are applied to speakers in noisy environments such as those in VoxCeleb2 because most of the TTS and VC algorithms assume high-quality and clean data. 
We adopt a method referred to as {\em ``copy synthesis''}~\cite{PaulTaylor}, which utilises the vocoder, the last component of common TTS and VC systems, to create spoofed data. %We use the vocoder, the last component of common TTS and VC systems, to create spoofed data through ``copy synthesis''~\cite{PaulTaylor}. 
We used the code released by \cite{Wang2023a} and built four neural vocoders: HiFiGAN \cite{Kong2020}, WaveGlow \cite{prenger2018waveglow}, neural source-filter model (NSF) \cite{wang2018neural}, and NSF combined with a HiFiGAN discriminator. 
These vocoders were trained on the VoxCeleb2 development set and used to copy synthesize the training data for phase 2. 



% \section{Multi-stage training scheme}
% \label{sec:multistage}
% % The proposed training scheme includes between one to three phases, which consist of either of the two techniques to be explained in Sections \ref{ssec:sid} and \ref{ssec:cs}, or adopts both of them. 
% Figure~\ref{fig:SASV} illustrates the overall proposed SASV framework. As shown in Figure~\ref{fig:SASV} training scheme is divided into three stages: speaker identification-based pre-training, multi-task training with copy-synthesis data, and end-to-end SASV fine-tuning. Each training stage is defined in the following sub-sections.

% \subsection{Stage~1: Speaker identification-based pre-training}
% \label{ssec:sid}
% In order to compensate for the lack of data to train a single SASV system, VoxCeleb2~\cite{chung2018voxceleb2}, a large-scale speaker recognition dataset can be utilised. VoxCeleb2 development data only contains bona fide utterances from ~6k speakers. 
% %In stage~1, the SASV embedding network is pre-trained on VoxCeleb data by optimising the equal-weighted summation of the AAM softmax~\cite{deng2019arcface} and the angular prototypical~\cite{chung2020defence} objective functions.
% After pre-training stage, SASV embeddings are fine-tuned with both bona fide and spoofed utterances in stage~2.

% \subsection{Stage~2: Copy synthesis training}
% \label{ssec:cs}
% Training data generated from a variety of text-to-speech (TTS) synthesis and voice conversion (VC) algorithms, is a prerequisite for constructing single integrated SASV models. Nonetheless, building various TTS and VC systems is a technically demanding and time-consuming process. It also requires high-quality training data. To avoid this, a recent study~\cite{Wang2023a} explored the neural network based vocoders to do copy-synthesis on bon fide utterances to generate spoofed data.
% We used a similar idea to generate the copy-synthesis of VoxCeleb2 and ASVspoof 2019 LA training dataset. We employ four different types of neural vocoders as described in~\cite{Wang2023a}: HiFiGAN~\cite{Kong2020}, WaveGlow~\cite{prenger2018waveglow}, neural source-filter model (NSF) \cite{wang2018neural}, and NSF with a HiFiGAN discriminator. A vocoder takes acoustic features such as F0 and mel spectrogram as input and produces the speech waveforms.\\

% While the acoustic features in TTS and VC are predicted from acoustic models given input text or source speech, for copy-synthesis, we extract (i.e., copy) the acoustic features from a target waveform and reconstruct (i.e., synthesise) the waveform.  Even though the copy-synthesised waveforms cannot encode the artefacts caused by acoustic models, they capture the vocoder's artefacts that might present in the spoofed data from the TTS and VC systems. The copy-synthesis data was found to be effective for spoofing CM~\cite{wu2013synthetic,Saratxaga2016,Wang2023a, sun2023exposing}. This set of vocoders covers flow, GAN, and differentiable digital signal processing techniques \cite{engel2020ddsp}. Furthermore, they generate waveforms at a real-time speed, making them ideal for copy-synthesis on a large data set. We use the copy synthesised data combined with corresponding bona fide data in stage~2. The model is trained using a combination of contrastive and identification loss functions described in Section~\ref{sec:loss}.

% % \subsection{Phase 3: fine-tuning}
% \subsection{Stage~3: Fine-tuning}
% \label{ssec:ft}
% In stage~3, we perform fine-tuning using in-domain bona fide and spoofed data from ASVspoof 2019 LA training dataset to improve generalisation. Stage~3 uses a similar training scheme and objective loss functions as stage~2.

% This phase adopts the identical training mechanism to phase 2: we use the combination of different objective functions which  detailed in Section~\ref{sec:loss}.

% We employ four types of neural vocoders released by \cite{Wang2023a}: HiFiGAN \cite{Kong2020}, WaveGlow \cite{prenger2018waveglow}, neural source-filter model (NSF) \cite{wang2018neural}, and NSF with a HiFiGAN discriminator.
% The task can become more challenging if the original (i.e., bona fide) data is not clean; the majority of TTS and VC algorithms assume high-quality clean data.
% they are applied to speakers in noisy environments such as those in VoxCeleb2 because most of the TTS and VC algorithms assume high-quality and clean data. 
% We adopt a method referred to as {\em ``copy synthesis''}~\cite{PaulTaylor}, which utilises the vocoder, the last component of common TTS and VC systems, to create spoofed data. %We use the vocoder, the last component of common TTS and VC systems, to create spoofed data through ``copy synthesis''~\cite{PaulTaylor}. 
% We used the code released by \cite{Wang2023a} and built four neural vocoders: HiFiGAN \cite{Kong2020}, WaveGlow \cite{prenger2018waveglow}, neural source-filter model (NSF) \cite{wang2018neural}, and NSF combined with a HiFiGAN discriminator. 
% These vocoders were trained on the VoxCeleb2 development set and used to copy synthesize the training data for phase 2. 
% %\textcolor{red}{how the data is used for Phsae 2...}

%% old table1 results descrption 













% % EFFECT OF PHASE1
% % First, a comparison of the first to third rows demonstrates that pre-training speaker identity using a large number of bonafide utterances can help the model discriminate target and non-target trials. %as long as they are all bona fide.
% % Fine-tuning the model in phase 3 can further help the model to discriminate spoofed trials (SPF-EER 22.38\% to 2.28\% for SKA-TDNN) with relatively less sacrifice in SV-EER. 
% % By using VoxCeleb bonafide in pre-training, the improvement of SV EER is notable and it leads to a reduction of SASV EER.
% % More interestingly, SPF EER is even decreased to approximately half which supports the fact that the spoofing detection task is correlated to speaker verification directly.

% % EFFECT OF PHASE2
% Second, comparison of rows 2, 4, and 8 show that Phase 2 (i.e., CS training with proposed loss functions) can be a substitute of phase 1. 
% Phase 2 can also complement Phase 1 which comparing rows 2, 4, and 6 discovers.
% % This may indicate that CS has unique features that include spoofing clues but are distinct from the spoof information in ASVspoof data.
% When adopting only phases 2 and 3, applying phase 2 with VoxCeleb2 and VoxCeleb2-CS was more effective than ASVspoof2019 bona fide and ASVspoof2019LA-CS.
% It may signify that, because phases 2 and 3 use the same loss functions, CS data, which only includes artefacts coming from vocoders, does not contain additional information when actual spoofed data, which includes artefacts coming from both acoustic model and vocoders, is available. 
% % The utilisation of copy synthesis data lead to large improvements in all performance of SASV, SV and SPF EERs,
% % compared to the case of using only VoxCeleb bonafide data.
% % From the results of using only VoxCeleb bonafide and copy synthesis, the performance is exactly in between the baseline and VoxCeleb bonafide only.
% % Noticeably, the combined results of VoxCeleb bonafide and copy synthesis data show the best performance in most cases. 
% % Lastly, the ASVspoof copy synthesis results show that the scale and SV EER have a large impact on overall performance.

% %EFFECT OF COMINBING ALL PHASES1 TO 3.
% Row 7, which leverages all three phases, demonstrated the best result, where in MFA-Conformer trained with both train and development partitions of ASVspoof2019LA in phase 3 shows SASV-EER of 1.06\%.
% This result outperforms the existing state of the art single integrated SASV model by a large margin.
% % In summary, the proposed pre-training scheme and the use of copy synthesis data demonstrate their effectiveness in learning speaker and spoof information, respectively.

==> nickSection2.tex <==
The proposed single, integrated framework and multi-stage training scheme is depicted in Figure~\ref{fig:SASV}.  Each stage is described below.

%Training is divided into three stages: speaker identification-based pre-training, multi-task training with copy-synthesis data, and end-to-end SASV fine-tuning. Each training stage is defined in the following sub-sections.

\subsection{Stage~1: Speaker identification-based pre-training}
\label{ssec:sid}

Reliable ASV systems require training using massive databases containing data collected from many thousands of speakers. 
Since none of the ASVspoof databases contain such sufficient data, we use the 
VoxCeleb2~\cite{chung2018voxceleb2}, a large-scale speaker recognition database, for speaker identification pre-training.
It contains bona fide utterances collected from ~6k speakers. 
Pre-training is performed by optimising the equal-weighted summation of additive angular margin (AAM) softmax~\cite{deng2019arcface} and angular prototypical~\cite{chung2020defence} objective functions.

%After pre-training stage, SASV embeddings are fine-tuned with both bona fide and spoofed utterances in stage~2.

\subsection{Stage~2: Copy-synthesis training}
\label{ssec:cs}

The training of CMs also requires huge databases of both spoofed and bona fide data. 
While bona fide data is available in abundance, the generation of spoofed data can be technically demanding and time-consuming, especially when the scenario involves spoofed utterances generated using text-to-speech (TTS) synthesis and voice conversion (VC) algorithms.
Critically, in order to protect generalisation, spoofed training data should also be generated with a wide variety of different spoofing algorithms. 
An efficient means to generate massive databases for spoofing CM training was proposed recently~\cite{Wang2023a}.
It uses neural network based vocoders and a copy-synthesis (CS) technique to generate spoofs from bona fide utterances using oracle acoustic features 
(e.g.\ F0 and mel spectrogram representations), and speaker embeddings (e.g.\ x-vectors). \\
 
 Similar ideas have been applied to create CS spoofs~\cite{wu2013synthetic,Saratxaga2016, pal2018synthetic, frank2021wavefake, sun2023exposing}, even though most of the previous studies use traditional non-neural vocoders.
We adopt the same idea and use CS spoofs generated using VoxCeleb2 and ASVspoof 2019 LA training datasets. 
We employ the same four neural vocoders as in the original work~\cite{Wang2023a}: HiFiGAN~\cite{Kong2020}; WaveGlow~\cite{prenger2018waveglow}; a neural source-filter model (NSF)~\cite{wang2018neural}; a NSF model with a HiFiGAN discriminator. 
%The copy-synthesis data was found to be effective for spoofing CM~\cite{wu2013synthetic,Saratxaga2016,pal2018synthetic,frank2021wavefake,Wang2023a, sun2023exposing}. 
This set of vocoders includes flow, generative adversarial network (GAN), and differentiable digital signal processing techniques~\cite{engel2020ddsp}, and can generate waveforms at real-time speed, making them ideally suited to CS using large datasets. 
%We use the copy synthesised data combined with corresponding bona fide data in stage~2. 
The model is trained using a combination of contrastive and identification loss functions described in Section~\ref{sec:loss}.



% \subsection{Phase 3: fine-tuning}
\subsection{Stage~3: Fine-tuning}
\label{ssec:ft}
Fine-tuning is performed using in-domain bona fide and spoofed data contained within the ASVspoof 2019 LA training partition.  
While training data corresponds to the same domain as that used for evaluation, there are differences in the spoofing algorithms used in their generation.
Stage~3 uses a similar training scheme and objective loss functions as stage~2.


==> old_loss_function_section.tex <==
\section{Objective functions}
\label{sec:loss}
This section describes different objective functions used in multi-stage training.

\subsection{ASV loss function}
In stage~1, the SASV embedding network is pre-trained on VoxCeleb data by optimising the ASV objective loss function defined in Eq.~(\ref{eq:ASV_loss}). Given a mini-batch of SASV embeddings, $\textbf{x}_{i,1}$ and $\textbf{x}_{i,2}$, where $\textbf{x}_{i,k}$ denotes a SASV embedding extracted from the $k^{\text{th}}\in [1,2]$ utterance of the $i^{\text{th}} \in [1,..,C_{\text{spk}}]$ speaker, we define support and prototype SASV embeddings as $\textbf{x}_{i,1}$ and $\textbf{x}_{i,2}$, respectively.
The angular prototypical~\cite{chung2020defence} loss function is defined as follows:
\begin{gather}
\mathcal{L}^{\text{asv}}_{\text{ap}} = -{1 \over N} \sum_{i}^{N} \log {\exp(f(\textbf{x}_{i,1},\textbf{x}_{i,2}))  \over {{\sum_{j}^{N}} \exp(f(\textbf{x}_{i,1},\textbf{x}_{j,2}))}},
\end{gather}
where $N$ is the number of speakers within a mini-batch and $f(\cdot)$ is a cosine similarity function with trainable scale and bias parameters.

Furthermore, we combine the angular prototypical loss with the AAM softmax~\cite{deng2019arcface} loss which has shown more competitive performance than using as alone~\cite{mun2023frequency}. %hi sunghwan can you confirm one thing in slack?
Given a target speaker label $\textbf{y}_{i,k}=i\in[1,..,C_{\text{spk}}]$ corresponding to $\textbf{x}_{i,k}$, AAM softmax loss is defined as:
\begin{gather}
  \mathcal{L}^{\text{asv}}_{\text{aam}} = \text{AAMsoftmax}(\textbf{x}_{i,j}, {\textbf{y}}_{i,j}; C_{\text{spk}}) \\
  = -{1 \over 2N} \sum_{i,k}^{2N} \log { e^{s\cos(\theta_{\textbf{y}_{i,k}, i}+m)}  \over {e^{s\cos(\theta_{\textbf{y}_{i,k},i}+m)} + \sum_{j \neq \textbf{y}^{c}_{i,k}} e^{s\cos(\theta_{j, i})}}},
\end{gather}

where $s$ is a scale factor, $m$ is a margin, $\text{cos}(\theta_{j,i})$ is the normalized dot product between the weight for the $j^{\text{th}} \in [1,..,C^{\text{spk}}]$ class and the input SASV embedding $\textbf{x}_{i,k}$.

Finally, the ASV loss function for stage~1 training is defined as the equal-weighted summation of two objective functions:
\begin{gather}
  \mathcal{L}^{\text{asv}} = \mathcal{L}^{\text{asv}}_{\text{ap}} + \mathcal{L}^{\text{asv}}_{\text{aam}}.
  \label{eq:ASV_loss}
\end{gather}

\subsection{SASV contrastive loss function}
\label{ssec:contrastive}
The angular prototypical loss used in stage~1 can maximise speaker discrimination between the embeddings from
different speakers. However, in the case of a spoof-aware scenario, this may affect (degrade) the overall performance as this objective loss does not take into account the CM label (i.e., spoof, target bona fide). Therefore we explore a contrastive loss function for single, integrated SASV training, and multi-stage training schemes that includes copy synthesis data.

Given a mini-batch of support and prototype SASV embeddings, $\textbf{x}^{c}_{i,1}$ and  $\textbf{x}^{c}_{i,2}$, where $\textbf{x}^{c}_{i,k}$ denotes a SASV embedding extracted from the $k^{\text{th}}\in [1,2]$ utterance of the $i^{\text{th}} \in [1,..,C_{\text{spk}}]$ speaker with CM label $c \in [\text{bna}, \text{spf}]$.
The spoofing-aware speaker verification contrastive loss is defined as follows:

\begin{gather}
  \mathcal{L}^{\text{sasv}}_{\text{cont}} = -{1 \over N_{\text{bna}}} \sum_{i}^{N_{\text{bna}}} \log {\exp(f(\textbf{x}^{\text{bna}}_{i,1},\textbf{x}^{\text{bna}}_{i,2}))  \over {{\sum_{j,c}^{N}} \exp(f(\textbf{x}^{\text{bna}}_{i,1},\textbf{x}^{c}_{j,2}))}},
\end{gather}
where $N_{\text{bna}}$ is the number of bona fide speakers within a mini-batch and $N=N_{\text{bna}}+N_{\text{spf}}$ indicates the total number of bona fide and spoof speakers within a mini-batch.

In stage~2, to focus more on the differences in the artefacts derived from the vocoders than other variations (e.g., speakers, phonetic characteristics, etc.), we construct the mini-batch such that the bona fide and corresponding copy-synthesised utterances are included together.

Given a bona fide utterance, $\textbf{x}^{\text{bna}}_{i,k}$, its copy synthesised data is denoted by $\textbf{x}^{\text{cs}}_{i,k}$.
We configure a mini-batch with a size of $2N_{\text{spk}}$ as follows: $\{[(\textbf{x}^{\text{c}}_{i,1},\textbf{x}^{\text{c}}_{i,2})]_{i,c}|\forall i\in [1,..,N_{\text{spk}}], \forall c\in [\text{bna}, \text{cs}]\}$, where the vocoder type used for copy synthesis is randomly selected.

In stage~3, we randomly sample the $2N_{\text{spk}}$ bona fide and $2N_{\text{spf}}$ spoofed data from the spoofing dataset, i.e., ASVspoof 2019 LA~\cite{wang2020asvspoof} training partition, without any restrictions.

% In stage~2, to focus more on the differences in the artefacts derived from the vocoders than other variations (e.g., speakers, phonetic characteristics, etc.), we construct the mini-batch such that the bona fide and corresponding copy-synthesised utterances are included together.
% % Given a bona fide utterance with a length of $T$, $\textbf{x}^{\text{bna}}_{i,k;[1:T]}$, its copy synthesised data is denoted by $\textbf{x}^{\text{cs}}_{i,k;[1:T]}$.
% Given a bona fide utterance, $\textbf{x}^{\text{bna}}_{i,k}$, its copy synthesised data is denoted by $\textbf{x}^{\text{cs}}_{i,k}$.
% We configure a mini-batch with a size of $2N_{\text{spk}}$ as follows: $\{[(\textbf{x}^{\text{c}}_{i,1},\textbf{x}^{\text{c}}_{i,2})]_{i,c}|\forall i\in [1,..,N_{\text{spk}}], \forall c\in [\text{bna}, \text{cs}]\}$, where the vocoder type used for copy synthesis is randomly selected.
% In stage~3, we randomly sample the $2N_{\text{spk}}$ bona fide and $2N_{\text{spf}}$ spoofed data from the spoofing dataset, i.e., ASVspoof 2019 LA~\cite{wang2020asvspoof} training partition, without any restrictions.

% \subsection{SASV identification loss functions}
% \label{ssec:identification}
% The SASV task can be considered as a multi-task problem where it needs to distinguish between target and non-target speakers, as well as bona fide and spoof.
% We investigate two approaches; (1) integrated SASV identification (i.e., $C_{\text{spk}}+1$ class classification) where all the spoofed conditions are considered as an additional class and (2) multi-task SASV identification (i.e., $C_{\text{spk}}$ speaker classification and binary spoofing detection tasks).




\subsection{SASV loss}
\label{ssec:identification1}
% For given bona fide and spoof SASV embeddings, $\textbf{x}^{\text{bna}}_{i,k}$ and $\textbf{x}^{\text{spf}}_{i,k}$, we set their corresponding SASV identification targets to $\textbf{y}^{\text{bna}}_{i,k}=i\in[1,..,C_{\text{spk}}]$ and $\textbf{y}^{\text{spf}}_{i,k}=C_{\text{spk}}+1$, respectively.


% where $\hat{\textbf{y}}^{c}_{i,k}=i\in[1,..,C_{\text{spk}}]$ and $\tilde{\textbf{y}}^{c}_{i,k}=c\in[\text{bna, spf}]$ are speaker and CM labels for SASV embedding $\textbf{x}^{c}_{i,k}$, respectively. $\alpha$ and $\beta$ are a weighting factor for each task.
The SASV task can be considered as a multi-task problem where it needs to distinguish between target and non-target speakers, as well as bona fide and spoof.
We investigate two approaches; (1) integrated SASV identification (i.e., $C_{\text{spk}}+1$ class classification) where all the spoofed conditions are considered as an additional class and (2) multi-task SASV identification (i.e., $C_{\text{spk}}$ speaker classification and binary spoofing detection tasks).\\

\newpara{Integrated SASV identification loss}
\label{ssec:identification1}
For given bona fide and spoof SASV embeddings, $\textbf{x}^{\text{bna}}_{i,k}$ and $\textbf{x}^{\text{spf}}_{i,k}$, we set their corresponding SASV identification targets to $\hat{\textbf{y}}^{\text{bna}}_{i,k}=i\in[1,..,C_{\text{spk}}]$ and $\hat{\textbf{y}}^{\text{spf}}_{i,k}=C_{\text{spk}}+1$, respectively.
To formulate $C_{\text{spk}}+1$ class identification objective, we exploit the AAM softmax~\cite{deng2019arcface} loss as follows:
% \begin{align}
%   & \mathcal{L}^{\text{sasv}}_{\text{id}_1} = \text{AAMsoftmax}(\textbf{x}^{c}_{i,k}, {\textbf{y}}^{c}_{i,k}; C_{\text{spk}}+1) \\
%   & = {-1 \over 2N} \sum_{i,k,c}^{2N} \log { e^{s\cos(\theta_{\textbf{y}^{c}_{i,k}, i}+m)}  \over {e^{s\cos(\theta_{\textbf{y}^{c}_{i,k},i}+m)} + \sum_{j \neq \textbf{y}^{c}_{i,k}} e^{s\cos(\theta_{j, i})}}},
% \end{align}
\begin{equation}
  \mathcal{L}^{\text{sasv}}_{\text{id}_1} = \text{AAMsoftmax}(\textbf{x}^{c}_{i,k}, {\hat{\textbf{y}}}^{c}_{i,k}; C_{\text{spk}}+1).
\end{equation}
where $\text{cos}(\theta_{j,i})$ is the normalized dot product between the weight for the $j^{\text{th}} \in [1,..,C^{\text{spk}}+1]$ class and the input SASV embedding $\textbf{x}^{c}_{i,k}$.\\


\newpara{Multi-task SASV identification loss}
\label{ssec:identification2}
Instead of learning the SASV embeddings from an integrated single output logit, a multi-task learning~\cite{caruana1998multitask} framework can be utilised. With $C_{\text{spk}}$ speaker classifier and binary spoofing detector, multi-task SASV identification loss is obtained as follows:
\begin{align}
  &\mathcal{L}^{\text{sv}}_{\text{id}_2} = \text{AAMsoftmax}(\textbf{x}^{c}_{i,k}, {\textbf{y}}^{c}_{i,k}; C_{\text{spk}}), \\
  &\mathcal{L}^{\text{spf}}_{\text{id}_2} = \text{AAMsoftmax}(\textbf{x}^{c}_{i,k}, \tilde{\textbf{y}}^{c}_{i,k}; 2), \\
  &\mathcal{L}^{\text{sasv}}_{\text{id}_2} = \mathcal{L}^{\text{sv}}_{\text{id}_2} + \mathcal{L}^{\text{spf}}_{\text{id}_2},
\end{align}
where ${\textbf{y}}^{c}_{i,k}=i\in[1,..,C_{\text{spk}}]$ and $\tilde{\textbf{y}}^{c}_{i,k}=c\in[\text{bna, spf}]$ are speaker and CM labels for SASV embedding $\textbf{x}^{c}_{i,k}$, respectively. 
% $\alpha$ and $\beta$ are a weighting factor for each task.
